BPMR: Bayesian Probabilistic Multivariate Ranking

Multi-aspect user preferences are attracting wider attention in recommender systems, as they enable more detailed understanding of users' evaluations of items. Previous studies show that incorporating multi-aspect preferences can greatly improve the performance and explainability of recommendation. However, as recommendation is essentially a ranking problem, there is no principled solution for ranking multiple aspects collectively to enhance the recommendation. In this work, we derive a multi-aspect ranking criterion. To maintain the dependency among different aspects, we propose to use a vectorized representation of multi-aspect ratings and develop a probabilistic multivariate tensor factorization framework (PMTF). The framework naturally leads to a probabilistic multi-aspect ranking criterion, which generalizes the single-aspect ranking to a multivariate fashion. Experiment results on a large multi-aspect review rating dataset confirmed the effectiveness of our solution.

==> old_intro.tex <==
\section{Introduction}
With the intention to comprehend user's detailed preferences beyond merely overall preference for items, multi-aspect preferences are extensively collected and become easily available online. Previous studies have shown that incorporating such multi-aspect preferences in addition to overall preference can greatly boost the performance of preference prediction and ranking, and promote the explainability of the recommendation \cite{EFM, Diao:2014:JMA:2623330.2623758, multiverse, bptf, HongImproving}. On the other hand, low-rank factorization methods have demonstrated its natural fitness and effectiveness in collaborative filtering based algorithms \cite{PMF, Marlin:2004:MMF:1015330.1015437}, which are broadly applied for recommendations\cite{Koren:2009:MFT:1608565.1608614, DBLP:journals/corr/abs-1802-07839}. These factors altogether make tensor factorization (TF) one of the most popular approaches to multi-aspect preference modeling \cite{TensorDecomp, MTER, multiverse, tagRec}. The idea behind TF based models is that each slice of the tensor corresponds to the preference matrix of an aspect. The properties of users, items and aspects can be represented by latent factor matrices as $U\in \mathbb{R}_+^{M\times d^U}$, $V\in \mathbb{R}_+^{N\times d^V}$, $W\in \mathbb{R}_+^{K\times d^W}$ respectively, where $M,\,N,\,K$ are the numbers of users, items, aspects and $ds$ are the dimensions of latent factors used to represent them. Then the prediction of each element in the resulting tensor could be measured by the distance of latent factor vectors in the joint latent space defined by a specific tensor factorization method as $X_{uil} =<U, V, W>_{uil}$. The predicted aspect preferences are usually used as explanations to support overall preference \cite{MTER, HongImproving, EFM}. However, from a probabilistic view of tensor factorization \cite{PMF, Rai:2015:SPT:2832747.2832775, bptf, temporal}, almost all of them simply assume that the multi-aspect preferences are independently given by expressing the likelihood of observing the multi-aspect preferences as point-wise product:
\begin{equation}
    p(R|U,V,W,\sigma^2) = \prod\limits_{u=1}^M\prod\limits_{i=1}^N\prod\limits_{l=1}^K \big[\mathcal{N}(r_{uil}|<U,V,W>_{uil},\sigma^2)\big]^{I_{uil}}
\label{eq:ptf}
\end{equation}
where $I_{uil}$ is the indicator of observing the aspect preference $r_{uil}$ \footnote{If not specified, the overall preference is treated as one of the aspects.}. This point-wise estimation criterion will lead to potential inconsistency in the prediction of the overall preference and the associated aspect preferences, which also contradicts to the original aspiration of explanation \cite{viewpoint, MTER, EFM}. %Figure \ref{fig:inconsistency} shows an example of such inconsistency in recommending hotels. I am afraid we do not have enough space for a figure
For instance, given the ground truth overall rating and one associated aspect rating of a user-item pair being $(4, 4)$ and they are positively correlated, we have two predictions of $(3,5)$ and $(5,5)$, where $(5,5)$ is apparently preferred for the consistency in prediction and explanation. But the point-wise estimation criterion cannot tell the difference between them because the defined probabilistic objective is equivalent to imposing the loss of square error to the ratings in this observation independently. %As a good explanation is to support the predicted overall preference which is used for recommendation \cite{MTER}, the inconsistency issue will also make the predicted aspect preferences fail this goal.

Although there has been impressive success in rating prediction tasks, arguably, the recommendation is essentially a ranking problem \cite{MTER,Sun2017MRLRMR}. Ranking criterion such as Bayesian personalized ranking (BPR) \cite{BPR,Sun2017MRLRMR} is proposed and widely adopted to directly optimize the preference ranking, in which the objective is to maximize the probability of observed orders. Nevertheless, previous works are only designed for single-aspect ranking which can only be applied to overall preference or to each aspect separately. The problem of ranking multiple aspects collectively remains unsolved, where the challenge is to design a ranking criterion that enables multi-aspect comparison.

By taking a holistic view of the generation of multi-aspect data, it is necessary to take a vectorized representation of all aspect ratings from a user to an item and view the vector as a integrated observation of preference. This new perspective makes it possible to model the intrinsic dependency among aspects and such dependency is also an indicator for generating explanations. Based on the limitations in handling the multi-aspect preference data discussed above, we propose a probabilistic tensor factorization framework with multivariate Gaussian distribution (PMTF) for describing the generation of the aspect ratings as $\bm R_{ui} \sim \mathcal{N}(<U,V,W>_{ui}, \Sigma_{ui})$, $\bm R_{ui}\in \mathbb{R}^K$. From an information-theoretic perspective \cite{l2x, Kullback1959Information}, we will show that by including the correlations, our framework provides information-theoretic guarantees for the consistency and explainability. 

With the proposed framework, we derive a Bayesian probabilistic multivariate ranking criterion (BPMR), which considers the comparison between observed pair-wise orders of vectors collectively. In original BPR, the probability of pair-wise order is obtained by converting the difference of two predicted preference levels to $(0,1)$ with a mapping function $p(i >_u j) := \sigma(\hat x_{ui} - \hat x_{uj})$. However, our solution directly optimizes the probability of the observed pair-wise orders of vectors, and thus optimize the ranking of all aspects simultaneously.

In Section 2 and 3, we derive the detailed formulation of the framework and the ranking criterion. In Section 4, a specific EM algorithm is proposed to learn both the latent factors and covariance matrices. We show in section 5 that both quantitative and qualitative experiment results on a large TripAdvisor multi-aspect dataset demonstrate the effectiveness of our framework. Experimental comparisons between our proposed probabilistic ranking criterion and existing methods show the improved performance of our solution.  

==> old_method.tex <==
\section{Probabilistic Multivariate Tensor Factorization}
\label{pmtf}
Suppose we have $M$ users, $N$ items and $K$ features, and preferences are indicated by explicit ratings. Instead of being an independent scalar as in previous works \cite{PMF, Rai:2015:SPT:2832747.2832775}, each observation is a vector of aspect ratings for item $i$ given by user $u$, denoted as $R_{ui} = (r_{ui1}, r_{ui2}, ..., r_{uiK})$. We use $\bm R_{ui}$ to denote the random vector from which $R_{ui}$ is generated. For simplicity, we use CP Decomposition as a specific tensor factorization method to illustrate our framework, where three matrices $U\in\mathbb R_+^{M\times d}$, $V\in\mathbb R_+^{N\times d}$, $W\in\mathbb R_+^{K\times d}$ are used to represent latent factors of users, items and aspects, respectively, with each row vector representing a single entity. The predicted aspect ratings are then obtained as $\hat R_{ui} = (U_u * V_i)W^T$, where $*$ denotes the element-wise product. 
\subsection{Proposed Framework}
We assume the aspect ratings are correlated in each observation and apply multivariate Gaussian to model the joint distribution of each aspect rating vector. The correlations constructed from the learnt covariance matrix can serve as indicators for generating explanations. We first impose a global covariance matrix for all user-item pairs for analysis, and will later enable personalized covariance matrix with Item Response Theory. Then the conditional distribution over the observed aspect rating vectors is
\begin{equation}
    p(R|U,V,W,\bm\Sigma_G) = \prod\limits_{u=1}^M\prod\limits_{i=1}^N\big[\mathcal{N}(R_{ui}|(U_u * V_i)W^T, \bm\Sigma_G)\big]^{I_{ui}}
\end{equation}
where $\mathcal{N}(\bm{x}|\bm{\mu}, \bm\Sigma)$ is the probability density function of the multivariate Guassian distribution with mean $\bm \mu$ and covariance matrix $\bm\Sigma$. $I_{ui}$ is an indicator function which is $1$ if user $u$ rated item $i$ and $0$ otherwise. The covariance matrix is no longer a hyperparameter to be set, but important statistics to be revealed from the observations. To let the parameters be conditioned on the observations, we place zero-mean spherical Gaussian priors on three latent factor matrices $U,V,W$ \cite{PSMF, PMF}:
\begin{equation}
    p(U|\sigma_U^2) = \prod\limits_{u=1}^M \mathcal{N}(U_u|0,\sigma_U^2 \bm I) 
\end{equation}
the priors for $V, W$ are similar. We impose the normal-inverse-Wishart distribution which is defined on real-valued positive (semi)definite matrices as the prior for the covariance matrix \cite{Conjugate,wishart}:
\begin{equation}
    p(\bm\Sigma|\Psi,\nu) = \frac{|\Psi|^{\nu/2}}{2^{\nu K/2}\Gamma_K(\frac{\nu}{2})}|\bm \Sigma|^{-(\nu + K + 1)/2}e^{\frac{1}{2}tr(\Psi\bm\Sigma^{-1})}
\end{equation}
where $|X|$ is the determinant of a matrix $X$ and $tr(X)$ is the trace of $X$. $\nu$ and $\Psi$ are hyperparameters which mean that the prior covariance matrix was estimated from  $\nu$ observations and with sum of pairwise deviation products $\Psi$. Then the log of the posterior distribution over all latent factors and the covariance matrix is:
\begin{equation}
\begin{split}
   \mbox{ln}\,p(U,&V,W,\bm\Sigma_G|R,\nu,\Psi,\sigma_U^2,\sigma_V^2,\sigma_W^2) \\
    = &-\frac{1}{2} \sum\limits_{u=1}^M\sum\limits_{i=1}^N I_{ui} \big[(R_{ui} - (U_u*V_i)W^T)\bm\Sigma_G^{-1}(R_{ui} - (U_u*V_i)W^T)^T +\mbox{ln}|\bm\Sigma_G|\big] \\ 
    & -\frac{\nu +K+1}{2}\mbox{ln}|\bm\Sigma_G| + \frac{1}{2}tr(\Psi\bm\Sigma_G^{-1}) + \frac{\nu}{2}\mbox{ln}|\Psi| - \mbox{ln}\,2^{\nu K/2}\Gamma_K(\frac{\nu}{2}) \\ 
    & + \mbox{ln}\,p(U|\sigma_U^2) + \mbox{ln}\,p(V|\sigma_V^2) + \mbox{ln}\,p(W|\sigma_W^2) + C
\end{split}
\label{eq:posterior}
\end{equation} 
where $\mbox{ln}\,p(U|\sigma_U^2) = -\frac{1}{2}(\frac{1}{\sigma_U^2}\sum\limits_{u=1}^MU_uU_u^T + Md\,\mbox{ln}\sigma_U^2)$, and similar for $V$ and $W$. $C$ is a constant that does not depend on the parameters. Note that there might be missing aspect ratings in $R_{ui}$, and we can simply apply a binary indicator vector $\bm I_{ui}\in \mathbb{R}^K$ to the difference between the observed and predicted aspect rating vector in equation \eqref{eq:posterior} as $(R_{ui} - (U_u*V_i)W^T)*\bm I_{ui}$. 

\paragraph{Information-Theoretic Interpretation} One important benefit of introducing correlations among aspect ratings is to enhance the explainability of making recommendations, where correlations are indicators of which aspects (explanatory variables) to select for explaining the overall preference prediction (response variable). Chen et al. \cite{Chen:2017:KFS:3295222.3295438} propose to minimize the trace of the conditional covariance operator and select features that maximally account for the dependence of the response on the covariates. The idea is similar to our strategy of selecting aspects with highest correlations with overall preference for explanation. Chen et al. \cite{l2x} interpret the explainability from an information-theoretic perspective, that the mutual information between the response variable and the explanations should be maximized. It turns out that the term involving the covariance matrix in the log likelihood in equation \eqref{eq:posterior} is consistent with such information-theoretic interpretations, which provides a lower bound to the mutual information among all aspects. Specifically, we have:
\paragraph{Theorem 1.}Given the variance vector of K random variables $\bm\sigma = (\sigma_{x1}, \sigma_{x2}, \dots , \sigma_{K})^T$, the mutual information of $K$ multivariate variables $\bm X \in \methbb R^K$ with covariance matrix $\bm\Sigma$ is lower bounded by $-\mbox{ln}|\bm\Sigma|$:
\begin{equation}
    I(\bm X) \geq -\frac{1}{2}\mbox{ln}|\bm\Sigma| + C
\end{equation}
with equality holds when the one variable is correlated with the other variables while the correlations among all other variables are $0$. \\
\textit{proof:} The covariance matrix could be written as $\bm\Sigma = (\bm\sigma\bm\sigma^T)*\bm\rho$, where $\bm\rho$ is the correlation matrix constructed from $\bm\Sigma$. With Hadamard product, we have:
\begin{equation*}
    det(\bm\Sigma) = det((\bm\sigma\bm\sigma^T)*\bm\rho) \geq det(\bm\sigma\bm\sigma^T)\cdot det(\bm\rho)
\end{equation*}
\begin{equation*}
    \mbox{ln}|\bm\Sigma| \geq \mbox{ln}|\bm\sigma\bm\sigma^T| + \mbox{ln}|\bm\rho|
\end{equation*}
It has been proved that $I(\bm X) = -\frac{1}{2}\mbox{ln}|\bm\rho|$ \cite{mutualinfo}, which leads to
\begin{equation*}
    \mbox{ln}|\bm\Sigma| \geq \mbox{ln}|\bm\sigma\bm\sigma^T| - 2I(\bm X)
\end{equation*}
\begin{equation*}
    I(\bm X) \geq -\frac{1}{2}\mbox{ln}|\bm\Sigma| + C
\end{equation*}
The proof of equality is postponed to Appendix A. Theorem 1 means that maximizing the likelihood under the proposed framework introduced an information-theoretic regularization term that indirectly maximize the mutual information. More specifically, when the correlation only happens between the overall preference and aspect preference, while all aspect preferences are independent, the term with $-\mbox{ln}|\bm\Sigma|$ is exactly equivalent to the mutual information. Such information-theoretic interpretation confirmed the rationale of our design and guarantees the explainability of predicted aspect ratings in the proposed framework.

\subsection{Personalized Covariance Matrix with Item Response Theory}
In previous discussion, a global covariance matrix is shared among all user-item pairs. The global covariance will tend to reveal the general correlations among aspects over the whole population of users and items. However, the emphasis of different users on aspects may vary, and the same logic applies to items. Therefore, the covariance matrix should be personalized for users and items to capture their detailed preferences, and the observed vector should follow the covariance matrix composed with corresponding user and item personalized covariance. To formally model the personalized covariance composition for the observation of a user-item pair, we take a perspective stemmed from the Item Response Theory (IRT) \cite{Fayers2004Item,Reid2007Modern}. IRT is originally from psychometrics, which states that the probability of a specific
response is determined by the item’s attribute and the subject’s individuality \cite{Lin}. Mapping back to our problem, we assume that the covariance matrix of the observation is a result of two independent channels of preference emphasis from the corresponding user and item. Specifically, we assign each user i and each item j a personalized covariance matrix $\bm\Sigma_i^U$ and $\bm\Sigma_j^V$. Then the covariance matrix of a pair of user-item is given by:
\begin{equation}
    \bm\Sigma_{ui} = \lambda\bm\Sigma_u^U + (1-\lambda)\bm\Sigma_i^V
\end{equation}
where $\lambda \in [0,1]$ is set as a hyperparameter. Besides, the covariance matrix needs sufficient observations to estimate. For some users and items with only a few observations, it is intractable to estimate accurate covariance matrices. To address the problem of lacking enough observations for some users and items, we apply the global covariance matrix $\bm\Sigma_G$ learnt from equation \eqref{eq:posterior} as the prior of individual covariance matrices of users and items. So the personalized covariance matrices will be acquired by modifying the global covariance matrix with even a few observations. This leads to the log posterior distribution with personalized covariance matrices:
\begin{equation}
\begin{split}
    \mbox{ln}\,p(U,&V,W,\bm\Sigma|R,\nu,\Psi,\sigma_U^2,\sigma_V^2,\sigma_W^2) \\
    = &-\frac{1}{2} \sum\limits_{u=1}^M\sum\limits_{i=1}^N I_{ui} \big[(R_{ui} - (U_u*V_i)W^T)\bm\Sigma_{ui}^{-1}(R_{ui} - (U_u*V_i)W^T)^T +\mbox{ln}|\bm\Sigma_{ui}|\big] \\ 
    & +\sum\limits_{u=1}^M \big[-\frac{\nu+K+1}{2}\mbox{ln}|\bm\Sigma^U_u| + \frac{1}{2}tr(\Psi{\bm\Sigma_u^{U}}^{-1}) + \frac{\nu}{2}\mbox{ln}|\Psi| - \mbox{ln}\,2^{\nu K/2}\Gamma_K(\frac{\nu}{2})\big]\\ 
    & +\sum\limits_{i=1}^N \big[-\frac{\nu+K+1}{2}\mbox{ln}|\bm\Sigma^V_i| + \frac{1}{2}tr(\Psi{\bm\Sigma_i^{V}}^{-1}) + \frac{\nu}{2}\mbox{ln}|\Psi| - \mbox{ln}\,2^{\nu K/2}\Gamma_K(\frac{\nu}{2})\big]\\ 
    & + \mbox{ln}\,p(U|\sigma_U^2) + \mbox{ln}\,p(V|\sigma_V^2) + \mbox{ln}\,p(W|\sigma_W^2) + C
\end{split}
\label{eq:personalized-posterior}
\end{equation} 
where $\bm\Sigma$ represents the set of all covariance matrices, and $\Psi = \nu\bm\Sigma_G$. Directly maximizing \eqref{eq:personalized-posterior} corresponds to the prediction task, but from a multivariate perspective. However, ranking is believed to be the essential problem in recommendation. We will show how the proposed framework naturally leads to the derivation of a probabilistic multi-aspect ranking criterion in the next section. 

\section{Bayesian Probabilistic Multivariate Ranking}
\subsection{Reformulation of BPR}
The foundation of the original BPR optimization criterion (BPR-OPT) \cite{BPR} is to maximize the probability of observing ground-truth pair-wise orders of the overall preference. In order to formalize it, we need to first construct an order set $D_S: P\times Q\times Q$ by:
\begin{equation}
    D_S := \{(u,i,j)|i >_u j\}
\end{equation}
where $P$ is the set of all users and $Q$ the set of all items. The meaning of $(u,i,j) \in D_S$ is that user $u$ prefer item $i$ over item $j$. An assumption is made in BPR that observed items in a user's review history ($r>0$) are always preferred over unobserved items ($r=0$). Then the likelihood of observed pair-wise orders is formulated as:
\begin{equation}
    \prod\limits_{u\in P}p(>_u|\Theta) = \prod\limits_{(u,i,j)\in P\times Q\times Q} p(\bm r_{ui}>\bm r_{uj}|\Theta)^{\delta((u,i,j)\in D_S)}
    \cdot p(\bm r_{ui}>\bm r_{uj}|\Theta))^{\delta((u,i,j)\notin D_S)}
\label{eq:BPR}
\end{equation}
where $\delta(b)$ is an indicator function which is 1 if $b$ is true and 0 otherwise. $\bm r_{ui}$ is the random variable from which the observed preference $r_{ij}$ of user $u$ to item $i$ is generated. However, it is not feasible to define the order set for vectors of multi-aspect observations. To extend it to multi-aspect ranking criterion, we first rewrite the likelihood and get rid of $D_S$ by expressing the observed pair-wise order with the difference between two observed preferences:
\begin{equation}
    \prod\limits_{u\in P}p(>_u|\Theta) = \prod\limits_{(u,i,j)\in P\times Q\times Q}p((\bm r_{ui} -\bm r_{uj}) sign(r_{ui} -r_{uj}))>0|\Theta)
\label{eq:BPR-reform}
\end{equation}
In equation \eqref{eq:BPR-reform}, $sign(r_{ui} -r_{uj})$ takes $1$ or $-1$ to indicate the observed ordering of a pair of items $(i,j)$ for a specific user $u$. Furthermore, with explicit preferences such as numerical ratings, we can get rid of the $sign$ function to let the pair-wise orderings have different weights. So larger observed preference difference of a pair of items will lead to higher weights in the ranking objective. 

\subsection{Multi-aspect Ranking with PMTF}
For multi-aspect explicit preferences denoted as $R_{ui} = (r_{ui1},\dots,r_{uik})$ for user $u$ to item $i$, we can apply equation \eqref{eq:BPR-reform} to multi-aspect explicit preferences collectively:
\begin{equation}
\begin{split}
    \prod\limits_{u\in P}p(>_u|\Theta) &= \prod\limits_{(u,i,j)\in P\times Q\times Q}p(\sum\limits_{l=1}^K(\bm r_{uil} - \bm r_{ujl}) (r_{uil} - r_{ujl})>0|\Theta) \\
                &= \prod\limits_{(u,i,j)\in P\times Q\times Q}p((\bm{R}_{ui} -\bm{R}_{uj})\cdot ({R}_{ui} -{R}_{uj})>0|\Theta) \\
                %&= \prod\limits_{(u,i,j)\in P\times Q\times Q}p(\hat{\bm d}_{uij}\cdot\bm d_{uij}>0|\Theta)
\end{split}
\label{eq:multi-bpr}
\end{equation}
Here we assume all aspects are equally treated in the ranking criterion. But if there are difference emphasis for difference aspects, we can apply a weighting vector $\bm w\in \mathbb R^K$ and take the Hadamard product as: $(\bm{R}_{ui} -\bm{R}_{uj})\cdot(({R}_{ui} -{R}_{uj})*\bm w)$. For conciseness, we denote $\bm D_{uij} = \bm R_{ui} -\bm R_{uj}$ as a random vector from which the observed difference $D_{uij} = R_{ui} - R_{uj}$ is generated. 
%A dot product is taken between the two difference vectors, which has a natural illustration in the multi-aspect space as shown in Figure \ref{fig:diffdot-product}. 
In previous works, the probability defined on the difference between preferences is often obtained by a mapping function, such as the sigmoid \cite{BPR} or softmax \cite{Sun2017MRLRMR}. However, with PMTF proposed in section \ref{pmtf}, we can directly get the probability distribution of $\bm D_{uij}$ by assuming preferences to different items are independently given by a user:
\begin{equation}
    p(\bm D_{uij} = D_{uij}|U,V,W,\bm\Sigma) = \mathcal{N}(D_{uij}|(U_u * (V_i-V_j))W^T, \bm\Sigma_{uij})
\end{equation} 
where $\bm\Sigma_{uij} = \bm\Sigma_{ui} + \bm\Sigma_{uj}$. After taking the dot product of $\bm D_{uij}$ and $ D_{uij}$, it naturally leads to the explicit expression of \eqref{eq:multi-bpr}:
\begin{equation}
\begin{split}
    &\prod\limits_{u\in P}p(>_u|\Theta)
    = \prod\limits_{(u,i,j)\in P\times Q\times Q}p(\bm D_{uij}\cdot D_{uij}>0|\Theta) \\
    &= \prod\limits_{(u,i,j)\in P\times Q\times Q}\int_0^\infty p(\bm D_{uij}\cdot D_{uij}|\Theta)d\bm D_{uij}\cdot D_{uij} \\
    &= \prod\limits_{(u,i,j)\in P\times Q\times Q}\int_0^\infty \mathcal{N}(\bm D_{uij}\cdot D_{uij}|(U_u * (V_i-V_j))W^T \cdot D_{uij}, D_{uij}\bm\Sigma_{uij}D_{uij}^T)d\bm D_{uij}\cdot D_{uij} \\
    &= \prod\limits_{(u,i,j)\in P\times Q\times Q}\frac{1}{2}\Big[1 - erf(\frac{- (U_u * (V_i-V_j))W^T \cdot D_{uij}}{\sqrt{2}\sqrt{D_{uij}\bm\Sigma_{uij} D_{uij}^T}})\Big]
\end{split}
\label{eq:bpmr}
\end{equation}
where $erf(x)=\frac{2}{\sqrt\pi}\int_{0}^{x}e^{-t^2}dt$ is the error function. Taking the log of \eqref{eq:bpmr} and substitute it to the first term of \eqref{eq:posterior} and \eqref{eq:personalized-posterior} accordingly will give us the posteriors for Bayesian Probabilistic Multivariate Ranking criterion (see Appendix B).
%\begin{equation}
%\begin{split}
%    BPMF-OPT 
%    := &\sum\limits_{(u,i,j)\in P\times Q\times Q} \mbox{ln}\Big[1 - erf(\frac{- (U_u * (V_i-V_j))W^T \cdot D_{uij}}{\sqrt{2}\sqrt{D_{uij}\bm\Sigma_{uij} D_{uij}^T}})\Big] \\ 
%    & +\sum\limits_{i=1}^M \big[-\frac{\nu+K+1}{2}\mbox{ln}|\bm\Sigma^U_i| + \frac{1}{2}tr(\Psi{\bm\Sigma_i^{U}}^{-1}) + \frac{\nu}{2}\mbox{ln}|\Psi| - \mbox{ln}\,2^{\nu K/2}\Gamma_K(\frac{\nu}{2})\\ 
%    & +\sum\limits_{j=1}^N \big[-\frac{\nu+K+1}{2}\mbox{ln}|\bm\Sigma^V_j| + \frac{1}{2}tr(\Psi{\bm\Sigma_j^{V}}^{-1}) + \frac{\nu}{2}\mbox{ln}|\Psi| - \mbox{ln}\,2^{\nu K/2}\Gamma_K(\frac{\nu}{2})\\ 
%    & + \mbox{ln}\,p(U|\sigma_U^2) + \mbox{ln}\,p(V|\sigma_V^2) + \mbox{ln}\,p(W|\sigma_W^2) + C
%\end{split}
%\label{eq:bpmr}
%\end{equation}
Although the error function could not be expressed as elementary functions, the derivative of it is given by $\frac{d}{dx}erf(x)=\frac{2}{\sqrt\pi}e^{-x^2}$. Therefore we could easily apply gradient based methods to optimize the objective function.   

\section{Optimization}
As we want to reveal the underlying correlations among aspects, the covariance matrices could be treated as hidden values in the parameter learning procedure. Thus, we adopt an EM algorithm to learn both the latent factor matrices and the covariance matrices. In M-step, we perform stochastic gradient descent (SGD) to update latent factor matrices $U,V,W$. In E-step, we first update the global covariance matrix with SGD based on \eqref{eq:posterior}, and then use the global covariance matrix as a prior parameter for updating the personalized covariance matrices based on \eqref{eq:personalized-posterior}. The time complexity of training with SGD scaleOne iearly with the number of the size of the training set. mportant ths lins lining to note is that in order to learn valid covariance matrices, we need to ensure that they are symmetric and positive semi-definite \cite{covariance}. For the positive semi-definite constraint, we can simply apply $\bm\Sigma = LL^T$, where L is an arbitrary matrix with the same dimensionality $\mathbb R^{K\times K}$ of $\bm\Sigma$. Then for any non-zero column vector $\bm x$, we have $\bm x^TLL^T\bm x = (L^T\bm x)^T(L^T\bm x) \geq 0$, which proves the positive semidefinite property of $LL^T$. The symmetric property is naturally satisfied as $LL^T = (LL^T)^T$. With this decomposition of covariance matrix, we update $L$ in the optimization procedure and construct the covariance matrices with corresponding $L$. Derivatives with respect to all parameters based on \eqref{eq:posterior}, \eqref{eq:personalized-posterior} and \eqref{eq:bpmr} are provided in Appendix B.

The above learning algorithm is applicable generally to tasks based on PMTF. However, for the ranking task, we have in total $O(M\times N\times N)$ training triples of $(u,i,j)$, making it necessary to find an efficient sampling strategy for SGD. Follow the solution in \cite{BPR}, we adopt bootstrap sampling with replacement of training triples, which samples the triples in each iteration uniformly at random. As two unobserved items of a user will not give us any update, in practice, we first randomly sample a rating vector $R_{ui}$ from all observations, and then randomly sample another item $j$ from all items for the same user $u$. What needs to be emphasized is that full cycles through the data is not necessary any more, because there are massive overlaps in the training triples. For example, if we have $i>_uj$ and $j>_uk$, then $i>_uk$ is naturally satisfied based on transitivity of ordering. We choose the number of samples for each iteration linearly depending on the number of observations and often a fraction of all triples is sufficient for convergence. 




==> older_intro.tex <==
\section{Introduction}
%Researchers have proved that incorporating extra information beyond merely overall preference can greatly boost the performance of preference prediction and promote the transparency of the recommendation \cite{HFT, EFM, viewpoint}. The improved transparency is of cardinal significance for improving users' trust, which is fundamental in real-world deployments \cite{Sharma:2013:SEW:2488388.2488487, Sinha01beyondalgorithms:, Symeonidis2008Providing, Bilgic05explainingrecommendations:}. On the other hand, 
Low-rank factorization models have demonstrated its natural fitness and effectiveness in collaborative filtering based algorithms \cite{PMF, Marlin:2004:MMF:1015330.1015437}, which are broadly applied for recommendations and learning embeddings \cite{Koren:2009:MFT:1608565.1608614, DBLP:journals/corr/abs-1802-07839}. On the other hand, incorporating extra information beyond merely overall preference in factorization models have been proved to greatly boost the performance of preference prediction and can promote the explainability \cite{HFT, EFM, viewpoint, Diao:2014:JMA:2623330.2623758}. These factors altogether make tensor factorization one of the most popular approaches to multi-aspect preference prediction \cite{TensorDecomp, MTER, multiverse, tagRec}, with each slice of the tensor corresponding to the preference matrix of an aspect. The idea behind such kinds of models is that the properties of users, items and aspects can be represented by factors matrices as $U\in \mathbb{R}^{M\times d^U}$, $V\in \mathbb{R}^{N\times d^V}$, $W\in \mathbb{R}^{K\times d^W}$ respectively, where $M,\,N,\,K$ are the numbers of users, items, aspects and $ds$ are the dimensions of latent factors used to represent them. Then the prediction of each element in the resulting tensor could be measured by the distances of latent factor vectors in the joint latent space defined by a specific tensor factorization method as $X_{ijl} =<U, V, W>_{ijl}$ (some tensor factorization methods also include extra components such as the core tensor in Tucker Decomposition). Compared to matrix factorization methods, tensor factorization alleviates the sparsity issue by including more information in assistance to the overall preference and the preference predictions of aspects are usually used as explanations of the resulting overall preference \cite{MTER, HongImproving}.  

In order to perform factorization based methods to large-scale sparse data, probabilistic factorization methods are proposed \cite{PMF,Rai:2015:SPT:2832747.2832775,Salakhutdinov:2008:BPM:1390156.1390267}, which are flexible in modeling different perspectives and scale linearly to the size of the training data. However, almost all of them by default assume that the preferences are independently given by expressing the likelihood of observing data as point-wise products: 
\begin{equation}
    p(R|U,V,W,\sigma^2) = \prod\limits_{i=1}^M\prod\limits_{j=1}^N\prod\limits_{l=1}^K \big[\mathcal{N}(R_{ijl}|<U,V,W>_{ijl},\sigma^2)\big]^{I_{ijl}}
\end{equation}
where $I_{ijl}$ is the indicator of observing preference $R_{ijl}$.
%and then impose proper priors to the latent factors, resulting in a Bayesian probabilistic model for latent factor learning. 
In the explanation phase of these point-wise estimation models, the explanatory aspects are usually chosen based on some heuristic rules such as the top rated aspects or user's most cared aspects. Such explanations are not necessarily explaining the generation of the final decision based on overall preferences. Besides, the point-wise estimation criterion will also lead to inconsistency in the prediction of the overall preference and the associated aspect preferences, which contradicts to the original aspiration of explanation. For example, given the ground truth overall rating and one associated aspect rating of a pair of user-item being $(4, 4)$ and they are positively correlated, and we have two predictions of $(3,5)$ and $(5,5)$, where $(5,5)$ is apparently preferred for the consistency in prediction and explanation. But the point-wise estimation criterion cannot tell the difference between them because the defined probabilistic objective is equivalent to imposing the loss of square error to the ratings in this observation independently. The reasons that these methods report better performance than matrix factorization on the prediction tasks might benefit from the better learnt latent factors with more data.  

By taking a holistic view of the generation of multi-aspect data, we argue that the preferences of all aspects for a pair of user-item should be correlated and considered as a vector of whole observation and there should not be independent assumptions. Therefore, we consider a probabilistic tensor factorization framework with multivariate Gaussian distribution (PMTF) with proper priors for describing each vector of observed aspect ratings as $R_{ij} \sim \mathcal{N}(R_{ij}|<U,V,W>_{ij}, \Sigma_{ij})$, $R_{ij}\in \mathbb{R}^K$. Similar to feature selection \cite{Chen:2017:KFS:3295222.3295438}, the correlations will capture the internal dependency of aspect ratings and serve as indicators of generating explanations. From an information-theoretic view of addressing explainability \cite{l2x, Kullback1959Information}, we will show that by including the correlations, our framework provides information-theoretic guarantees for the explainability. The traditional PTF falls into a special case of our framework by ignoring the correlations. We propose an EM algorithm to learn both the latent factors and covariance matrices with a vector-based probabilistic model and enable personalized correlations with the item-response theory \cite{Lin, Fayers2004Item}. 

Although impressive performance has been achieved on preference prediction tasks and almost reach its limits in recent years, the recommendation is essentially a ranking problem \cite{MTER, Sun2017MRLRMR}. Solutions for optimizing the ranking is proposed \cite{BPR, Shi:2010:LLR:1864708.1864764} to improve the top-n ranking performance, where the objective is to maximize the probability of observed orders. Nevertheless, previous works can only handle single-aspect ranking, i.e., the overall preference ranking, and the probability of pair-wise order is obtained by converting the difference of two preference levels to $(0,1)$ with a mapping function $p(i >_u j) := \sigma(\hat x_{ui} - \hat x_{uj})$. A straightforward thought is to rank each aspect separately with the single-aspect ranking criterion, but such strategies will potentially degenerate the ranking of other aspects when ranking a single aspect. Thus the problem of ranking multiple aspects collectively remains unsolved, where the challenge is to treat each vector of observation as a whole object in the ranking criterion. Based on the proposed framework, we derive a Bayesian probabilistic multivariate ranking criterion, which directly optimizes the probability of the observed pair-wise orders of vectors, and thus optimize the ranking of all aspects simultaneously. Both quantitative and qualitative experiment results demonstrate the effectiveness of our framework. Experimental comparisons between our proposed probabilistic ranking criterion and existing methods show the improved performance of our solution.  


